NyayaAnumana & INLegalLlama: The Largest Indian Legal Judgment Prediction Dataset and Specialized Language Model for Enhanced Decision Analysis

The integration of artificial intelligence (AI) in legal judgment prediction (LJP) has the potential to transform the legal landscape, particularly in jurisdictions like India, where a significant backlog of cases burdens the legal system. This paper introduces NyayaAnumana, the largest and most diverse corpus of Indian legal cases compiled for LJP, encompassing a total of 7,02,945 preprocessed cases. NyayaAnumana, which combines the words "Nyay" (judgment) and "Anuman" (prediction or inference) respectively for most major Indian languages, includes a wide range of cases from the Supreme Court, High Courts, Tribunal Courts, District Courts, and Daily Orders and, thus, provides unparalleled diversity and coverage. Our dataset surpasses existing datasets like PredEx and ILDC, offering a comprehensive foundation for advanced AI research in the legal domain. In addition to the dataset, we present INLegalLlama, a domain-specific generative large language model (LLM) tailored to the intricacies of the Indian legal system. It is developed through a two-phase training approach over a base LLaMa model. First, Indian legal documents are injected using continual pretraining. Second, task-specific supervised finetuning is done. This method allows the model to achieve a deeper understanding of legal contexts. Our experiments demonstrate that incorporating diverse court data significantly boosts model accuracy, achieving approximately 90% F1-score in prediction tasks. INLegalLlama not only improves prediction accuracy but also offers comprehensible explanations, addressing the need for explainability in AI-assisted legal decisions.

==> Ablation_study.tex <==
% \section{Ablation Study}
% In our ablation study, we investigated the impact of various court-level training data configurations on the performance of our models in the binary classification judgment prediction task. We observed consistent trends across multiple experiments, particularly when analyzing the results from the full Nyayanuman dataset in relation to subsets that excluded specific court cases. The performance metrics are detailed in Appendix Tables \ref{tab:binary-judgment-results-single-SCI-HCs-Tribunal}, \ref{tab:binary-judgment-results-multi-SCI-HCs-Tribunal}, \ref{tab:binary-judgment-results-single-SCI-HCs}, \ref{tab:binary-judgment-results-multi-SCI-HCs}, \ref{tab:binary-judgment-results-single-SCI}, \ref{tab:binary-judgment-results-multi-SCI}, \ref{tab:binary-judgment-results-ILDC-single}, and \ref{tab:binary-judgment-results-ILDC-multi}. 

% Our findings indicate that models trained on High Court cases exhibited the best performance, likely due to the substantial representation of High Court data in the training set. However, when these models were evaluated on the ILDC dataset, a noticeable drop in performance was observed, as shown in Appendix Tables \ref{tab:binary-judgment-results-ILDC-single-HCs} and \ref{tab:binary-judgment-results-ILDC-multi-HCs}. This suggests that while the models excel in familiar contexts, they struggle to generalize to datasets with different characteristics or distributions.

% We also conducted experiments on the ternary judgment prediction task, incorporating additional court cases, with results presented in Appendix Tables \ref{tab:judgment-prediction-ternary-sci-HCs}, \ref{tab:judgment-prediction-ternary-sci-hcs-tribunals}, and \ref{tab:judgment-prediction-ternary-sci-hcs-tribunals-dailyorders}. These experiments further reinforced the significance of including diverse court data and highlighted the benefits of utilizing large volumes of training data. 

% Our findings emphasize the importance of a diverse and comprehensive dataset. Including a broad spectrum of court cases not only enhances the model's understanding of various judicial contexts but also significantly improves its performance metrics. In particular, the models trained on the most extensive datasets achieved an F1 score of around 90\%, underscoring the critical role of data diversity and volume in achieving high accuracy.

% Overall, the ablation study illustrates that the diversity and volume of training data play a crucial role in enhancing model performance, particularly in the context of legal judgment prediction tasks. Future work should continue to explore the impact of various data configurations to further optimize model accuracy and generalization capabilities.

